Estimation of Electric Vehicle Public Charging Demand using Cellphone Data and Points of Interest-based Segmentation

The race for road electrification has started, and convincing drivers to switch from fuel-powered vehicles to electric vehicles requires robust Electric Vehicle (EV) charging infrastructure. This article proposes an innovative EV charging demand estimation and segmentation method. First, we estimate the charging demand at a neighborhood granularity using cellular signaling data. Second, we propose a segmentation model to partition the total charging needs among different charging technology: normal, semi-rapid, and fast charging. The segmentation model, an approach based on the city's points of interest, is a state-of-the-art method that derives useful trends applicable to city planning. A case study for the city of Brussels is proposed.

==> content/backup.tex <==
% %% Previous Figures
% \begin{figure}[!ht] \small
% \begin{centering}
%   \begin{minipage}[t]{0.40\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/neighborhoods-chant d'oiseau.png} 
%     \subcaption{\small The map highlights \textit{Chant d'Oiseau}, a heavily residential neighborhood, as shown by the numerous blue lines indicating a high proportion of housing. Regarding public amenities, it only accommodates a few shops. The PPR rate is relatively high due to the district's topology. \href{https://rawcdn.githack.com/victor-radermecker/BrusselsEVS35/de9ea9b64cdebacd508292d16a903faa889c2510/img/neighborhoods-chant-oiseau.html}{\textsc{Interactive Figure \faGithub}}} 
%     \label{ChantD'oiseau}
%   \end{minipage}%%
%     \qquad
%     \begin{minipage}[t]{0.40\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/neighborhoods-matonge.png}
%     \subcaption{\small The map highlights \textit{Matonge}, a neighborhood accommodating many public amenities such as bars and restaurants as well as shops. The high number of blue lines indicate a high proportion of housing (residential lanes). The PPR rate is very low due to the parking restrictions. \href{https://rawcdn.githack.com/victor-radermecker/BrusselsEVS35/88042091b57ba1b6f3d2e1e3765e7dec4ebecb47/img/neighborhoods-matonge.html}{\textsc{Interactive Figure \faGithub}}} 
%     \label{Matonge}
%   \end{minipage} 
%   \begin{minipage}[t]{0.40\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/neighborhoods-quartier-européen.png} 
%     \subcaption{\small The map highlights \textit{Quartier Européen}, a work district which accommodates many offices (especially the buildings of the European Institutions) and restaurants. This neighborhood also includes many long-term parking lots as people park their cars while their are at work. 
%     \href{https://rawcdn.githack.com/victor-radermecker/BrusselsEVS35/de9ea9b64cdebacd508292d16a903faa889c2510/img/neighborhoods-quartier-europ\%C3\%A9en.html}{\textsc{Interactive Figure \faGithub}}}
%     \label{Europe}
%     \vspace{1ex}
%   \end{minipage}%%
%     \qquad
%     \begin{minipage}[t]{0.40\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{img/neighborhoods - quartier royal.png} 
%     \subcaption{\small The map highlights \textit{Quartier Royal}, a touristic and work district. It includes many shops, boutiques, hotels and popular touristic spots. The residential ratio is substantially lower to other neighborhood and the heavy parking restrictions lead to an extremely low PPR. 
%     \href{https://rawcdn.githack.com/victor-radermecker/BrusselsEVS35/de9ea9b64cdebacd508292d16a903faa889c2510/img/neighborhoods-quartier-royal.html}{\textsc{Interactive Figure \faGithub}}} 
%     \vspace{1ex}
%     \label{Royal}
%   \end{minipage} 
%   \centerline{
%     \begin{minipage}[b]{0.75\textwidth}
%     \centerline{\includegraphics[width=0.75\linewidth]{img/mfe-icons3-2-legend.png}}
%     \end{minipage}}
%   \centerline{
%     \begin{minipage}[b]{0.75\textwidth}
%     \centerline{\includegraphics[width=0.75\linewidth]{img/mfe-icons3-3.png}}
%     \end{minipage}}
%     \caption{\small This figure shows four neighborhoods, each of them having a different nature. Their segmentation results are presented in \autoref{fig:segmentations-proportions}.}
%     \label{fig:segmentation_results}
% \end{centering}
% \end{figure}

==> content/literature_backup.tex <==
\section{Literature Review}
The literature abounds with articles on optimal locations of public EV charging stations. \autoref{independent} presents different studies which do not distinguish the different charging technologies.
These articles combine demand estimation methods with optimization models to derive the optimal locations of charging points. 
Although some papers are starting to emerge, very few authors have addressed roll-out strategies for different charging technologies. These are presented in \autoref{dependent}.

\subsection{Charging Type Independent Approaches}\label{independent}
As explained above, most authors have explored the problem of optimally locating charging stations without considering a specific technology between normal, semi-rapid and fast charging. Before applying any optimization algorithms, the first challenge is always to estimate the total charging demand.

\subsubsection{Demand Estimation}

Given its importance in optimization algorithms, demand estimation has been extensively examined by researchers worldwide. Many authors took advantage of Cellular Signaling Data (CSD) to estimate charging demand. Among them, \citeauthor{B1} proposed an approach to locate public charging stations using reconstructed EVs trajectories derived from simulation. The simulation is done through NEXTA, a mesoscopic simulation tool able to reconstruct a realistic trajectory based on multiple checkpoints. \cite{NEXTA} These checkpoints are activity locations, which are derived from CSD. When a driver's State of Charge (SOC), which is modeled by a linear relation, falls below a threshold, the energy consumed is assigned to the vehicle's geographic coordinates. Different clustering methods (DBSCAN, Hierarchical clustering, K-means, etc.) are then used to aggregate the demand.  \cite{B1} Although presenting promising results for Tianjin, this study requires CSD data at an individual level, which goes against the European GDPR (General Data Protection Regulations).   \\

% More advanced models for the driver's charging behavior
Whereas \citeauthor{B1} assumed a linear charging behavior for EV drivers, \citeauthor{B2} proposes a probabilistic mathematical model to simulate EV drivers’ charging habits. Many factors affect a driver’s charging needs, including the SOC, the next driving mileage, the travel time value, or even economic factors. \cite{B2}\\  

% Socio-Demographic factors
Socio-demographic factors are popular variables to model the charging demand. \citeauthor{B8} proposed to use institutional and spatial factors to Beijing's charging demand. They have identified six key socio-demographic attributes, namely income, vehicle ownership, educational level, age, gender, and family size. \cite{B8} \citeauthor{B17} used a similar approach for Lisbon, but they distinguished nighttime and daytime charging. Nighttime demand was derived using the number of cars per household whereas daytime demand was estimated from the volume of employment in each district. \cite{B17}  \\

% Traffic simulation models and travel surveys
Travel surveys and traffic simulation are also well explored methodologies. \citeauthor{B4} proposes an approach based on an OD study and traffic simulation models. They build a travel OD matrix for Thessaloniki using data collected by a broad phone survey, which recorded the daily trips of 5.000 residents. A traffic simulator is then used to simulate the trips between OD pairs and derive charging demand. \cite{B4} Similarly, \citeauthor{B6} take advantage of a household travel survey from the French Rhone Region to build an energy OD matrix for the city’s neighborhoods. \cite{B6} A routing API is used to compute the driving distance under real traffic conditions. The final energy supply matrix is computed through a consumption model called the VEHLIB library, a tool providing EV consumption estimation based on trips and altitude data \cite{B18} \cite{B19}. \citeauthor{Z2} took advantage of a geocoded mobility survey for the Coimbra, which questioned around 10,000 drivers about their daily trips on business days. They built an energy OD Matrix by converting these trips into EV consumptions under some specific assumptions. \cite{Z2}  \\

Finally, others used car-parking demand to establish the charging demand in urban areas. \citeauthor{D3} states that the charging demand is roughly proportional to the total parking duration for all light-duty vehicles. They aggregated a dataset of around 50 000 person trips and combined it to land use characteristics. Using this input data, they trained an Ordinary Least Squares (OLS) regression to ultimately predict the total parking times. \cite{D3}\\

% Optimization algorithms
\subsubsection{Optimization Models}

Once the charging demand is estimated, the use of optimization models allows locating optimal sites for stations. Many researchers, such as \citeauthor{B3}, have extensively aggregated the existing optimization models. \cite{B3}  \\

To name a few, \citeauthor{Z5} introduced a capacitated refueling location model (CRLM) to locate EV charging stations. The original uncapacitated model assumes that the presence of a refueling station is sufficient to supply all vehicles intersecting the station node, which was not realistic for EVs. This CRLM model limits the number of cars refueling at each station and introduces a new objective function that maximizes vehicle miles traveled instead of the number of trips. \cite{Z5} \citeauthor{Z2} proposed a mixed integer programming (MIP) model for locating charging stations in Coimbra. The model considers not only the drivers' parking locations but also their daily activities, which allows linking the charging demand to specific places. \cite{Z2} \\ 


% Find optimal locations
\citeauthor{B4} proposed a genetic algorithm approach to estimate the optimal location of charging stations. A value of 1 is assigned to the chromosome bits that have been selected for implementation of charging stations, while 0 are assigned to others. The advantage is that the algorithm provides valuable results with tiny datasets. \cite{B4} The authors of \cite{B5} have created an agent-based decision support system. Its end goal was to identify patterns in residential EV ownership as well as enable strategic deployment of new charging infrastructure. \citeauthor{Z6} have developed a simulation–optimization model which determines optimal EV charging stations location to maximize their use by privately owned EVs. A case study for the central-Ohio region demonstrates that mixing different charging technologies is preferable to only one type. \cite{Z6}  \\


\subsection{Charging Type Dependent Approaches}\label{dependent}

A few studies have focused on electric vehicle charging infrastructure for specific technologies. \citeauthor{D2} computed suitability scores for normal charging stations in urban areas. Their interesting approach relied on using Geographic Information System (GIS) data to determine the site suitability for hosting normal EV charging stations. By aggregating and analyzing various input factors such as land use, demographics, or employment centers, they were able to derive the suitability scores for each stations of the State of Utah (US). \cite{D2} Agent-based models have also been explored to investigate charging stations roll-out strategies for semi-rapid and fast technologies. \citeauthor{Z8} simulated a population of agents which included various profiles of drivers (citizens, foreigners, taxis, and shared vehicles) to exhaustively model the diversity of charging behaviors within cities. \cite{Z8} Regarding fast charging, \citeauthor{D1} investigated a widely accepted roll-out strategy, which consists of creating "electric corridors" on major interurban motorways to connect cities and towns. Their end goal was to assess the adequacy of this roll-out strategy, which in theory, should allow longer trips to be undertaken and, therefore, increase EV users' potential journey ranges. \cite{D1}  \\

% Optimization methods for specific cases.
Some authors have explored optimization methods for specific charging technologies. For instance, \citeauthor{Z7} have expanded the concepts of set-coverage and maximum-coverage to express a capacitated location model that deals with multiple types of charging stations, using a MIP algorithm. The main contributions of this study are that it relaxes the constraints of using a single kind of recharging station. The results highlight that a combination of charging technologies, although it requires a higher budget, leads to greater convenience for travelers. \cite{Z7} Others have also explored optimization models to locate charging stations for specific fleets, such as taxis, shared-cars and buses. \cite{Z3} \cite{Z4} \\


\subsection{A new approach}\label{new}

Consequently, numerous studies focus on estimating the total EV charging demand to apply location models. However, these approaches do not sufficiently account for the different charging technologies. This article proposes an innovative methodology, which, by segmenting the charging demand into various charging speeds, allows to re-use the technology-independent models presented in \autoref{independent} for specific charging speeds, and hence helps providing actionable insights to city planning authorities.  \\

Therefore, we present a two-step approach to segment the charging demand. First, we propose a demand estimation method, which does not rely on individual drivers' behavior and respects GDPR. Second, we take advantage of GIS data to assess each neighborhood's primary function and compute its needs for each charging types.  \\

The rest of the paper is structured as follows. Next, we present the methodology, which outlines our method to estimating and segmenting public charging demand. To illustrate our approach, we apply it to the case study of Brussels, Belgium. We present the datasets used and the various models. Results are summarized and discussed to highlight how they can provide actionable insights to planning authorities. Finally, we present conclusions of the work, identify limitations of this study, and present future areas for continued investigation. \\



% We can see that we have a lot of demand estimation methods available from literature to estimate. Segmenting this demand into charging type is something that was not explored, although it is super useful.

% As shown by the various examples above, many researchers have investigated the challenge of charging stations for electric vehicles, which is crucial to the electrification of our cities. However, the idea of segmenting the EV charging demand into several types of technologies (normal, semi-rapid, and fast) is not covered exhaustively by the existing literature.  

